MacGyver: Are Large Language Models Creative Problem Solvers?

We explore the creative problem-solving capabilities of modern LLMs in a novel constrained setting. To this end, we create MACGYVER, an automatically generated dataset consisting of over 1,600 real-world problems deliberately designed to trigger innovative usage of objects and necessitate out-of-the-box thinking. We then present our collection to both LLMs and humans to compare and contrast their problem-solving abilities. MACGYVER is challenging for both groups, but in unique and complementary ways. For instance, humans excel in tasks they are familiar with but struggle with domain-specific knowledge, leading to a higher variance. In contrast, LLMs, exposed to a variety of specialized knowledge, attempt broader problems but fail by proposing physically-infeasible actions. Finally, we provide a detailed error analysis of LLMs, and demonstrate the potential of enhancing their problem-solving ability with novel prompting techniques such as iterative step-wise reflection and divergent-convergent thinking. This work (1) introduces a fresh arena for intelligent agents focusing on intricate aspects of physical reasoning, planning, and unconventional thinking, which supplements the existing spectrum of machine intelligence; and (2) provides insight into the constrained problem-solving capabilities of both humans and AI.

==> tables/assess_difficulty.tex <==

\begin{table}[t]
\centering

\begin{subtable}{\columnwidth} %[] %[t]{\textwidth}
\centering
\scalebox{0.78}{
% \begin{table}[]
% \small\centering
\renewcommand{\arraystretch}{1.2}
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}ccccc@{}}
\toprule
  \textbf{Solutions} &
  \textbf{\begin{tabular}[l]{@{}l@{}}Feasible \\ \& eff. ($\uparrow$)\end{tabular}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}Feasible \\ \& ineff.\end{tabular}} &
  \textbf{\begin{tabular}[l]{@{}c@{}}Infeasible\\ ($\downarrow$)\end{tabular}} &
  \textbf{\begin{tabular}[l]{@{}l@{}}LLM says \\ unsolv. ($\downarrow$)\end{tabular}} \\ \midrule
 
Count & 247 & 555 & 490 & 14 \\
\rowcolor[HTML]{E7E6E6}
Percentage & 18.9\% & 42.5\% & 37.5\% & 1.1\% \\\bottomrule
\end{tabular}
}
\caption{Performance on the subset of the \DatasetName{} dataset that humans think is solvable.}
\label{table:result_sovable}
\end{subtable}
\vspace{-0.3em}

\begin{subtable}{\columnwidth} %[] %[t]{\textwidth}
\centering
\scalebox{0.78}{
\begin{tabular}{@{}cccc@{}}
\toprule
  \textbf{Answers} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Correct for\\ right reason ($\uparrow$)\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}Correct for \\ wrong reason\end{tabular}} &
  \textbf{\begin{tabular}[c]{@{}l@{}}LLM says \\ solvable ($\downarrow$)\end{tabular}} \\ \midrule
 
Count & 135 & 8 & 234 \\
\rowcolor[HTML]{E7E6E6}
Percentage & 35.8\% & 2.1\% & 62.1\% \\\bottomrule
\end{tabular}
}
\caption{Performance on the subset of the \DatasetName{} dataset that humans think is unsolvable. \textbf{Correct for right reason} means that the LLM correctly identifies the problem is unsolvable, and gives the right justification. \textbf{Correct for wrong reason} means that it correctly identifies the problem is unsolvable, but gives an incorrect justification.}
\label{table:result_unsovable}

\end{subtable}

\caption{GPT-4 performance on \DatasetName{} dataset. \violet{would it be better if we put them into a barchart where the total height of the bart is 1 (100\%), then different scenarios are color/pattern coded to show the percentage. like figure 2 in this page: \url{https://arxiv.org/pdf/1909.01326.pdf}} \faeze{I can give it a shot. Thou my only concern is that in here not all dimensions are "higher the better". So it might cause confusion?} \violet{it's actually the same situation in the paper I shared: positive higher the better, negative lower the better. You can probably use some colors/patterns convention to indicate. e.g., green means good, red means bad.} }\vspace{-3mm}
\vspace{-5mm}
\label{table:appendix-tools}
\end{table}
